Zone-based Federated Learning for Mobile Sensing Data

Mobile apps, such as mHealth and wellness applications, can benefit from deep learning (DL) models trained with mobile sensing data collected by smart phones or wearable devices. However, currently there is no mobile sensing DL system that simultaneously achieves good model accuracy while adapting to user mobility behavior, scales well as the number of users increases, and protects user data privacy. We propose Zone-based Federated Learning (ZoneFL) to address these requirements. ZoneFL divides the physical space into geographical zones mapped to a mobile-edge-cloud system architecture for good model accuracy and scalability. Each zone has a federated training model, called a zone model, which adapts well to data and behaviors of users in that zone. Benefiting from the FL design, the user data privacy is protected during the ZoneFL training. We propose two novel zone-based federated training algorithms to optimize zone models to user mobility behavior: Zone Merge and Split (ZMS) and Zone Gradient Diffusion (ZGD). ZMS optimizes zone models by adapting the zone geographical partitions through merging of neighboring zones or splitting of large zones into smaller ones. Different from ZMS, ZGD maintains fixed zones and optimizes a zone model by incorporating the gradients derived from neighboring zones' data. ZGD uses a self-attention mechanism to dynamically control the impact of one zone on its neighbors. Extensive analysis and experimental results demonstrate that ZoneFL significantly outperforms traditional FL in two models for heart rate prediction and human activity recognition. In addition, we developed a ZoneFL system using Android phones and AWS cloud. The system was used in a heart rate prediction field study with 63 users for 4 months, and we demonstrated the feasibility of ZoneFL in real-life.

==> sec1-intro-old.tex <==
\section{Introduction}

Sensing data collected on mobile devices can be employed in many novel Deep Learning (DL) applications. A practical application domain is mobile health and wellness, where data is collected by smart phones with potential help from wearable sensors. Such mobile apps require privacy protection and need to adapt to user behavior, which is location-dependent. For example, people's lifestyles depend on their living areas. Living in dense areas of the city with fewer recreational facilities prevents people from doing enough exercise. Low-income neighborhoods have less access to healthy food~\cite{hilmers2012neighborhood}. Some city neighborhoods are exposed to environmental pollution. Health/wellness apps using DL model can better predict users' health status with mobile sensing data incorporating user mobility behavior. 

An effective DL system for mobile sensing data needs to satisfy four requirements: (R1) achieve good model accuracy, (R2) adapt to user mobility behavior, (R3) scale well as the number of users increases, and (R4) protect user data privacy. Federated Learning (FL)~\cite{mcmahan2017fedAVG} is proposed as a solution to protect user data privacy. In FL, the models are trained on mobile devices with their local data, and the server aggregates the models received from mobile devices. The users' privacy-sensitive data never leave the mobile devices. Current FL solutions, however, do not address well the requirements for good model accuracy, adaptability to user mobility behavior, and good scalability. FL usually suffers from inferior model accuracy comparing with Centralized Learning(CL), because the on-device training is performed on non-Independent and Identically Distributed (non-IID) data. One key contributor to non-IID data distribution in FL is the user mobility behavior~\cite{hsu2007modeling}. To adapt to user mobility behavior, a naive approach in FL could be incorporate the user location as the model input. However, it will increase both the model size and computation overhead which occupy precious resources on mobile devices. The aggregation in FL relies on a central aggregation server, which limits its scalability. 

We propose \textbf{Zone-based FL (ZFL)} satisfying the four requirements associated with an effective DL system for mobile sensing data. The main idea of ZFL is to divide the space into a number of zones with similar user behaviors and train FL models for each zone. As users move from one zone to another, their mobile devices also switch from one zone model to another. In this way, ZFL adapts each zone model to the data and behaviors of the users who spend time in that zone, and achieves better accuracy (R1 and R2). ZFL system architecture can be deployed in a mobile-edge-cloud infrastructure, where edge nodes manage FL within the zones where these nodes are located. Edge nodes host the latest models for their zones, and mobile devices can download these models when they enter a new zone. The cloud dynamically keeps the zone partition information for the entire space. Compared to a mobile-cloud solution, a mobile-edge-cloud solution is more scalable (R3), has lower latency for mobile users, and results in less network bandwidth consumption in the network core~\cite{abbas2017Mobile-edge-survey2,murshed2019machineEdgeSurvey}. With the recent development of edge zones by public cloud providers such as Amazon AWS~\cite{aws-local-zones} and Microsoft Azure~\cite{azure-edge-zones}, ZFL can be deployed in real-life scenarios. ZFL protects privacy in the same way as vanilla FL because the data never leave the mobile devices (R4) . 
% For ZFL to work in a mobile-cloud solution, the users would need to share their zones with the cloud, which may lead to privacy concerns (i.e., the cloud may track users across zones).
Although each edge knows when a user has been in its zone, but it does not know when or how frequently a user has been in other zones. 

We propose two mechanisms for dynamic adaptation of zone partitions: Zone Merging and Splitting (ZMS) and Zone Gradients Diffusing (ZGD). In ZMS, zones dynamically merge and split during training. We apply a greedy algorithm to ensure merging and splitting will result in better model accuracy in each zone. ZMS can be used when the initial zone partition is suboptimal, and the zone partition will be gradually improved as ZFL proceeds. ZGD leverages the concept of graph neural networks. Each zone diffuses its gradients to its neighbors, and incorporates the gradients from its neighbors to achieve better model accuracy. ZGD can be used when the zone partition is pre-determined. For example, a smart city defines its zone based on administrative divisions. A cellular network provider partitions its zones based on the coverage of base stations. 

% To do

We implemented and evaluated two proof-of-concept applications with real-world datasets for ZFL. The first is heart rate prediction with FitRec dataset~\cite{ni2019modeling}. The second is Human Activity Prediction(HAR) with mobile sensing data collected in the wild. The experimental results demonstrate that ZFL leads to higher accuracy than global FL for zones that have enough training data. ZMS can effectively produce better zone partitions, while ZGD improves the best model accuracy. 
% ZMS can effectively produce better zone partitions in ?\% of the training rounds, while ZGD improves the best model accuracy by ?\%.  
We also implemented the two ZFL models with DL4J~\cite{dl4j} on Android and tested them on two phones. The results demonstrate that ZFL is feasible in practice. The two models achieve low training and inference latency, as well as low memory and battery consumption on the phones. Furthermore, the ZFL models are faster and consume fewer resources compared to the global FL models.

% XJ: On-device results above may be revised. ZFL on-device results may be higher than global FL (train 1/3 of data 3 times vs. train the whole data). Hopefully the overhead is not much. 

The rest of this paper is organized as follows. Section~\ref{sub:related} reviews the related work. Section~\ref{arch} presents the ZFL architecture.  Section~\ref{sub:algo} describes the algorithms for dynamic adaptation of zone partitions. Section~\ref{exp} shows the experimental results. The paper concludes in Section~\ref{con}. 




==> sec2_related_old.tex <==
\label{sec:related}

In this section, we briefly review federated learning, edge computing frameworks that support deep learning and clustering-based personalized FL. Based on that, we point of the differences between ZoneFL and these existing approaches.

\subsection{Federated Learning}

% FL is an intriguing DL framework for mobile sensing data at edge due to increasing privacy concerns from both regulations and general public~\cite{voigt2017eu,annas2003hipaa}.

Federated learning (FL) is a multi-round communication protocol instantiated between a coordination server and a set of $N$ clients to jointly train a parametrized learning  model $f_{\theta}$, e.g., a neural network, where $\theta$ is a vector of model parameters (also called weights). The training proceeds in rounds. At each round $t$ the server sends the latest model weights $\theta_t$ to a randomly sampled subset of clients $S_t$ (Figure \ref{FL Framework}). Upon receiving $\theta_t$, each client $u \in S_t$ uses $\theta_t$ to train its local model and generates model weights $\theta^u_t$. Client $u$
computes its local gradient $\nabla \theta^u_t = \theta^u_t - \theta_t$, and sends it back to the server. After receiving the local gradients from all the clients in $S_t$, the server updates the model weights by aggregating all the received local gradients using an aggregation function $\mathcal{G}: \mathbb{R}^{|S_t|\times n} \rightarrow \mathbb{R}^n$, where $n$ is the size of $\nabla \theta^u_t$. The aggregated gradient will be added to $\theta_t$: $\theta_{t+1} = \theta_t + \lambda \mathcal{G}(\{\nabla\theta^i_t\}_{i\in S_t})$, where $\lambda$ is the server’s learning rate. A typical and widely applied aggregation function $\mathcal{G}$ is the weighted averaging, dubbed Federated Averaging (FedAvg) \cite{kairouz2019advances}.

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=2.5in]{image/FL}
    \caption{Federated training protocol at a round $t$.}
    \label{FL Framework}
  \end{center}
\end{figure}

By joining a FL protocol, clients minimize the average of their loss functions as follows:
$\theta^* = \arg\min_\theta \frac{1}{N} \sum_{u = 1}^N L_u(\theta)$, where $L_u$ is the loss function of client $u$ on their local training dataset $D_u$, and defined as $L_u(\theta) = \frac{1}{|D_u|}\sum_{x \in D_u} L\big(f_{\theta}(x), y \big)$, where $|D_u|$ denotes the number of data samples in $D_u$, and $L$ is a loss function (e.g., cross-entropy) penalizing the mismatch between the predicted values $f_\theta(x)$ of an input $x$ and its associated ground-truth label $y$.

\subsection{Deep Learning at Edge} 

DL has been increasingly employed in edge computing for a broad range of autonomous operations and applications such as video analytics, speech recognition, fraud detection, and autonomous vehicles~\cite{Mledge1,Mledge2,lin2018Mledge3,Mledge4,Mledge5}. Most of works do not tackle the problem of privacy. Cui et al.~\cite{Stochastic} presented an online method to learn network changes and increase the network throughput. TinyDL~\cite{coffen2021tinydl} used acceleration data collected by finger-worn ring profile device to train a hand gesture recognition model with edge devices. Bouazizi et al.~\cite{bouazizi2022low} proposed using low-resolution infrared array sensors to identify the presence and location of people indoors with edge DL. These works simply offload data collected by a variety of sensors to edge computing, and can benefit from such a mobile sensing DL system as ZFL.

Several efforts have been carried out to leverage the computation power of both the cloud and the edge for DL. 
In~\cite{li2018learningIotinEdge}, the layers of a deep learning network are divided between edge servers and cloud, while~\cite{DistributedDeepNeural} proposed a distributed architecture over an edge-cloud infrastructure. Part of the models and tasks in these works are executed in the cloud. 

Departing from existing DL at edge systems, ZFL achieves better scalability as the entire training is distributed to mobile devices and edge nodes. The cloud only provides support for zone partition information.

\subsection{Clustering and Personalization in FL} 

To further improve the model accuracy of vanilla FL, user clustering has been proposed. Briggs et al.~\cite{briggs2020federated} presented a modification to FL with a clustering step to separate clusters of clients by the similarity of their local updates. Once separated, the clusters are trained independently. Similarly, clustered FL~\cite{sattler2020clustered} performs clustering, after FL has converged to a stationary point, with geometric properties of the FL loss surface. However, both of the works encounter the same scalability issue as vanilla FL, because they require a central entity to cluster users. Khan et al.~\cite{khan2020self} proposed a FL scheme with a clustering algorithm based on social awareness, and then a cluster head is selected to avoid using centralized cloud server. In~\cite{he2019single-sidedFederated}, users share their model parameters with a group of trusted friends. However, the utilizing social relationship carries extra privacy risks. 

Although sharing the idea of training models with groups of users, ZFL focuses on user mobility behavior, and does not require centralized user model updates or user information. ZFL also provides a solution that can be naturally deployed in cloud-edge-mobile infrastructure offering better scalability. That is one step forward compared with existing clustering-based FL approaches.

In addition to clustering-based FL, personalization in FL further mitigates non-iid data issue. The key idea of personalized FL is to learn a personalized model per user~\cite{mansour2020three}, which eliminates the challenge of user clustering without access to user data. There are different methods for adapting global models for individual users~\cite{kulkarni2020survey}, including adding user context, transfer learning, using personalized layers, knowledge distillation, etc. Ditto~\cite{li2021ditto} leverages global-regularized multi-task learning to provide fairness and robustness through personalization in FL.
In the adaptive personalized federated learning~\cite{deng2020adaptive}, each user trains a local model incorporating the global model with some mixing weights for the optimal combination. 
Ozkara et al.~\cite{ozkara2021quped} use quantization and distillation for personalized compression in FL by manipulating the loss function at the clients. Although effective, existing algorithms in personalized FL demand extra computation efforts from clients. That may affect their feasibility on resource constrained mobile devices. 

ZFL is orthogonal to model personalization in FL. In fact, existing personalized FL training techniques can be employed in ZFL to produce different models for each user in zones. However, evaluating personalized FL algorithms is not the focus of our study in this paper.


% Another aspect that makes Zone-FL broadly applicable is independence. ProtoNN \cite{gupta2017protonn} designed a prediction algorithm that could run on edge devices with limited resources. Nevertheless, ProtoNN generally has been devised to solve supervised learning problems. A similar Idea, Bonsai \cite{kumar2017Bonsai}, which is a resource-efficient tree-based algorithm, aims to minimize the model size while making a satisfactory prediction and using less memory and power. Unfortunately, as Bonsai presented to only work on tiny resource-limited devices, it is not comparable to such a deep neural network. MoDNN \cite{mao2017modnn} tries to tackle the training deep neural networks issues on mobile devices by a new model partitioning method. However, MoDNN required the data set to be on a group owner device and partitioned running tasks on worker nodes. Thus, it cannot solve the problem when each user needs to have its own data set, not a single shared data set.
